High-resolution ALMA observations of transition disk candidates in Lupus

Transition disks with small inner dust cavities are interesting targets for the study of disk clearing mechanisms. Such disks have been identified through a deficit in the infrared part of their SED, but spatially resolved millimeter imaging is required to confirm the presence of an inner dust cavity. We use high-resolution ALMA observations of 30 mas resolution in Band 6 continuum and $^{12}$CO 2--1 emission of 10 transition disk candidates in the Lupus star forming region, in order to confirm the presence of inner dust cavities and infer the responsible mechanism. The continuum data are analyzed using visibility modeling and the SEDs are compared with radiative transfer models. Out of the six transition disk candidates selected from their SED, only one disk revealed an inner dust cavity of 4 au in radius. Three of the other disks are highly inclined, which limits the detectability of an inner dust cavity but it is also demonstrated to be the possible cause for the infrared deficit in their SED. The two remaining SED-selected disks are very compact, with dust radii of only $\sim$3 au. From the four candidates selected from low-resolution images, three new transition disks with large inner cavities $>$20 au are identified, bringing the total number of transition disks with large cavities in Lupus to 13. SED-selected transition disks with small cavities are biased towards highly inclined and compact disks, which casts doubt on the use of their occurrence rates in estimating dispersal timescales of photoevaporation. Using newly derived disk dust masses and radii, we re-evaluate the size-luminosity and $M_{\rm dust}-M_{\rm star}$ relations. These relations can be understood if the bright disks are dominated by disks with substructure whereas faint disks are dominated by drift-dominated disks. (Abridged)

==> backup.tex <==
\begin{table}[!ht]
\centering
\caption{Properties $^{12}$CO line cubes}
\label{tbl:obsco}
\begin{tabular}{llll}
\hline
Target & Beam size & rms & SNR \\ 
&(")&(mJy km s$^{-1}$) \\
\hline
Sz76 & 0.19$\times$0.17 & 6.3 & 6 \\
Sz103 & -&-&- \\
Sz104 & -&-&- \\
Sz112 & -&-&- \\
J16011549 & 0.26$\times$0.23 & 5.6 & 21\\
J16081497 & -&-&- \\
J16000236 & 0.26$\times$0.23 & 5.0 & 14 \\
Sz129 & 0.26$\times$0.23 & 4.8 & 13 \\
J16090141 & 0.38$\times$0.36 & 12 & 10 \\
J16070384 & -&-&- \\
\hline
\end{tabular}
\end{table}


\begin{table}[!ht]
\footnotesize
\caption{MCMC best-fit parameters}
\label{tbl:mcmc}
\begin{tabular}{llllllllll}
\hline
Target	&	$\log I_0$	&	$r_c$	&	$\gamma_1$	&	$\gamma_2$	&	$i$	&	$PA$	&	dRA	&	dDec	   \\		
&(Jy sr$^{-1}$)&(")&&($\circ$)&($\circ$)&(")&(")\\
\hline
Sz76	&	10.44$^{+0.07}_{-0.19}$	&	0.031$^{+0.026}_{-0.018}$	&	0.81$^{+0.60}_{-0.46}$	&	1.00$^{+0.31}_{-0.23}$	&	66.31$^{+1.24}_{-1.47}$	&	85.60$^{+1.51}_{-1.43}$	&	-0.011$^{+0.002}_{-0.002}$	&	0.019$^{+0.001}_{-0.001}$			\\
Sz103	&	10.19$^{+0.07}_{-0.05}$	&	0.10$^{+0.002}_{-0.002}$	&	-0.17$^{+0.10}_{-0.08}$	&	5.70$^{+2.04}_{-1.49}$	&	66.13$^{+0.73}_{-0.74}$	&	-4.26$^{+0.90}_{-0.91}$	&	-0.005$^{+0.001}_{-0.001}$	&	0.029$^{+0.007}_{-0.007}$			\\
Sz104	&	10.23$^{+0.36}_{-0.23}$	&	0.024$^{+0.005}_{-0.005}$	&	-0.88$^{+0.52}_{-0.22}$	&	6.0 (fixed)	&	27.80$^{+12.39}_{-19.00}$	&	65.71$^{+26.93}_{-26.73}$	&	0.000$^{+0.000}_{-0.000}$	&	0.018$^{+0.001}_{-0.001}$			\\
Sz112	&	10.74$^{+0.11}_{-0.11}$	&	0.024$^{+0.002}_{-0.002}$	&	0.77$^{+0.51}_{-0.37}$	&	6.0 (fixed)	&	20.49$^{+8.53}_{-11.96}$	&	-32.91$^{+23.42}_{-24.99}$	&	0.003$^{+0.001}_{-0.001}$	&	0.019$^{+0.001}_{-0.001}$			\\
J16011549	&	8.59$^{+0.01}_{-0.01}$	&	0.97$^{+0.02}_{-0.02}$	&	-1.19$^{+0.004}_{-0.004}$	&	8.92$^{+1.93}_{-1.61}$	&	68.96$^{+0.44}_{-0.44}$	&	157.22$^{+0.52}_{-0.57}$	&	0.005$^{+0.000}_{-0.000}$	&	0.021$^{+0.000}_{-0.000}$			\\
J16081497	&	9.96$^{+0.11}_{-0.06}$	&	0.15$^{+0.01}_{-0.01}$	&	-0.28$^{+0.15}_{-0.09}$	&	3.55$^{+0.91}_{-0.91}$	&	78.29$^{+0.53}_{-0.59}$	&	84.84$^{+0.59}_{-0.57}$	&	0.002$^{+0.001}_{-0.001}$	&	0.017$^{+0.001}_{-0.001}$			\\
J16000236	&	9.51$^{+0.01}_{-0.01}$	&	0.64$^{+0.004}_{-0.004}$	&	-0.59$^{+0.01}_{-0.01}$	&	3.86$^{+0.15}_{-0.14}$	&	65.52$^{+0.19}_{-0.20}$	&	161.25$^{+0.23}_{-0.24}$	&	0.004$^{+0.001}_{-0.001}$	&	0.029$^{+0.001}_{-0.001}$			\\
Sz129	&	10.31$^{+0.02}_{-0.02}$	&	0.24$^{+0.01}_{-0.01}$	&	0.06$^{+0.02}_{-0.02}$	&	1.70$^{+0.04}_{-0.04}$	&	30.79$^{+0.41}_{-0.41}$	&	149.17$^{+0.74}_{-0.79}$	&	0.021$^{+0.001}_{-0.001}$	&	0.037$^{+0.001}_{-0.001}$			\\
\hline
	&	$\log I_r$	&	$r_r$	&	$r_w$	&	&	$i$	&	$PA$	&	dRA	&	dDec		\\
&(Jy sr$^{-1}$)&(")&(")&&($\circ$)&($\circ$)&(")&(")\\
\hline
J16090141	&	9.49$^{+0.04}_{-0.04}$	&	0.405$^{+0.003}_{-0.003}$	&	0.037$^{+0.003}_{-0.003}$	&	-	&	76.20$^{+0.31}_{-0.29}$	&	176.83$^{+0.25}_{-0.21}$	&	-0.005$^{+0.001}_{-0.001}$	&	0.020$^{+0.001}_{-0.001}$			\\
J16070384	&	8.77$^{+0.06}_{-0.06}$	&	0.17$^{+0.05}_{-0.08}$	&	0.16$^{+0.06}_{-0.05}$	&	-	&	77.82$^{+2.21}_{-2.71}$	&	147.05$^{+2.17}_{-2.20}$	&	-0.060$^{+0.020}_{-0.020}$	&	0.020$^{+0.030}_{-0.030}$		\\
\hline
\end{tabular}
\end{table}


\begin{table}[!ht]
\centering
\caption{Model properties}
\label{tbl:modelprop}
\begin{tabular}{llllll}
\hline
Target&Flux&$R_{\rm peak}$&$R_{90}$\\
&(mJy)&(au)&(au)\\
\hline
Sz76&2.7&4.0&25\\
Sz103&4.5&0&16\\
Sz104&1.0&0&3.5\\
Sz112&1.4&2.7&4.0\\
J16011549&23&0&129\\
J16081497&3.2&0&26\\
J16000236&50&0&106\\
Sz129&79&5.4&69\\
J16090141&4.1&64$^a$&74\\
J16070384&1.3&28&76\\
\hline
\end{tabular}\\
$^a$ This is the peak of the outer disk ring, the maximum in the image is the inner disk emission.
\end{table}

